MaskClustering: View Consensus based Mask Graph Clustering for Open-Vocabulary 3D Instance Segmentation

Open-vocabulary 3D instance segmentation is cutting-edge for its ability to segment 3D instances without predefined categories. However, progress in 3D lags behind its 2D counterpart due to limited annotated 3D data. To address this, recent works first generate 2D open-vocabulary masks through 2D models and then merge them into 3D instances based on metrics calculated between two neighboring frames. In contrast to these local metrics, we propose a novel metric, view consensus rate, to enhance the utilization of multi-view observations. The key insight is that two 2D masks should be deemed part of the same 3D instance if a significant number of other 2D masks from different views contain both these two masks. Using this metric as edge weight, we construct a global mask graph where each mask is a node. Through iterative clustering of masks showing high view consensus, we generate a series of clusters, each representing a distinct 3D instance. Notably, our model is training-free. Through extensive experiments on publicly available datasets, including ScanNet++, ScanNet200 and MatterPort3D, we demonstrate that our method achieves state-of-the-art performance in open-vocabulary 3D instance segmentation. Our project page is at https://pku-epic.github.io/MaskClustering.

==> fig/clustering_baselines.tex <==
\begin{figure}[htbp]
\centering
\begin{overpic}
[width=1\linewidth]
{fig/img/clustering.pdf}
\end{overpic}
\caption{
\textbf{Qualitative results of different clustering methods.} Clique-based clustering tends to over-segment, and single-time connected component-based clustering tends to under-segment. In contrast, our iterative clustering method yields perfect results.
}

% \vspace{-10pt}
\label{fig:clustering}
\end{figure}


==> fig/consensus_vs_geometry.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{fig/img/consensus_vs_geometry.pdf}
\caption{
\textbf{Case study.} Masks belonging to a same instance may display low geometric overlap but exhibit a high view consensus rate. The blue and red masks represent the side and frontal views, respectively, of the same armchair. Despite their low geometric overlap, both masks are visible in the rightmost frame and are contained by the same green mask, resulting in a high consensus rate.
}

% \vspace{-10pt}
\label{fig:consensus-vs-geometry}
\end{figure}

==> fig/geometry_failure.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\columnwidth]{fig/img/geometry.pdf}
\caption{
\textbf{Failure cases exemplifying over-segmentation in the geometric overlap-based method.} 
}

% \vspace{-10pt}
\label{fig:geometry}
\end{figure}

==> fig/geometry_pos_dis.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\columnwidth]{fig/img/Positive_geometry.pdf}
\caption{
\textbf{Distribution of Intersection over Union (IoU) for positive mask pairs}. 46.2\% of mask pairs belonging to the same instance exhibit low IoU, contributing to the over-segmentation phenomenon observed in the geometric overlap-based method.
}
\vspace{-10pt}
\label{fig:geometry_pos_dis}
\end{figure}

==> fig/hyper.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{fig/img/hyper.pdf}
\caption{
\textbf{Performance Variation with Changing Hyperparameters.}.
}

\label{fig:hyper}
\end{figure}

==> fig/semantic_dis.tex <==
\begin{figure}[htbp]
\centering
\begin{overpic}
[width=0.7\linewidth]
{fig/img/semantics.pdf}
\end{overpic}
\caption{
\textbf{Semantic Similarity Distribution for Positive and Negative Mask Pairs.} The distributions exhibit substantial overlap, indicating that negative pairs can possess high similarity, while positive pairs may exhibit low similarity. This overlap complicates the use of semantic similarity to reliably determine the relationship between two masks.
}

% \vspace{-10pt}
\label{fig:semantics_dis}
\end{figure}

==> fig/semantic_failure.tex <==
\begin{figure}[htbp]
\centering
\begin{overpic}
[width=1\linewidth]
{fig/img/semantic_failure.pdf}
\end{overpic}
\caption{
\textbf{Instances of Semantic Similarity Failures.} On the left, the side and frontal view of the same chair exhibit low similarity. On the right, all chairs in a room appear identical, causing different chairs to have high similarity.
}

% \vspace{-10pt}
\label{fig:semantic_failure}
\end{figure}

==> fig/supp_gallery.tex <==
\begin{figure*}[t]
\centering
\begin{overpic}
[width=1\linewidth]
%[width=\linewidth,grid,tics=10]
% {figure/image/gallery2.pdf}
{fig/img/supp_gallery.pdf}
\end{overpic}
\caption{
Comparison of 3D zero-shot segmentation performance. We compare our methods with OpenMask3D~\cite{takmaz2023openmask3d} and OVIR-3D~\cite{Lu2023OVIR3DO3} on ScanNet~\cite{dai2017scannet}.}
\label{fig:supp_gallery}
% \vspace{-10pt}
\end{figure*}


==> fig/teaser.tex <==
\begin{figure*}[t]
% \begin{teaserfigure}
% \centering
% \begin{overpic}
% [width=1\linewidth]
%[width=\linewidth,grid,tics=10]
% {figure/image/gallery2.pdf}
\includegraphics[width=\linewidth]{fig/img/teaser.pdf}
% \end{overpic}
\caption{
teaser}
\label{fig:teaser}
\end{figure*}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/useless.tex <==
% % \subsection{Mask back projection and under segment mask removal}
% For each frame t, we first obtain all $n_t$ candidate 2D masks $C_{(t,i)}, i=1,2,...,n_t$ in this frame. We then back-project these masks into the 3D world space and use ball query to get their corresponding points $P_{(t,i)}$ on the reconstructed mesh. Indices of these points are denoted as $I_{(t,i)}=\{j| p_j \in P_{(t,i)}\}$.

% We formulate the whole process as a graph building and clustering problem, where each node represents a mask and two nodes are connected only when they belong to a same instance. 

% % To judge whether two masks correspond to the same object, we examine them in the whole sequence. For two masks $C_{t_1,i_1}$ and $C_{t_2,i_2}$ \jiazhao{must form different view?}, if they are both visible in frame $t_3$, the visible part of $V_{t_1,i_1}$ should be contained by at least one mask $C_{t_3, i_3}$. 
% % Different from frame-to-model methods, our model doesn't heavily rely on geometric overlap. ???

% Meanwhile, we maintain a matrix $M \in R^{N \times T}$ where each N denotes the total vertice number of the reconstructed mesh and T denotes the total number of frames. Each cell $M[i,t]$ records the mask id that point $p_i$ belongs to in frame $t$. Note that masks are itemized from 1, so $M[i,t]=0$ means point $p_i$ is invisible in frame $t$. Note that the back-projected point cloud is not accurately aligned with the reconstructed mesh due to inaccuracy in camera poses and depth maps, so the radius of ball query should be large enough (3 $cm$ in practice), making nearby masks overlap on the same points sometimes. These points on the boundary may contribute to the geometry overlap between nearby masks, leading to excessive merging. Therefore, if a point $p_i$ is queried by two masks in a same frame, it is considered to be a boundary point and is removed by setting $M[i]=0$.\jiazhao{Dose this mean that some points will have not been considered as any mask?}

% For each candidate mask $C_{(t,i)}$, we can now efficiently find out all the frames it is visible in and all the masks it correspond to at these frames, denoted as $VF_{(t,i)}$ and $VM_{(t,i)}$. \jiazhao{Still confused. The column of $M$ if frame id, so how can you find the corresponding masks?} We can also filter out undersegment masks during this process. Given the high-quality nature of 2D segmentation models, in most views, different objects can be distinguished clearly. Therefore, if a candidate mask $C_{(t,i)}$ wrongly covers two objects in one view, $P_{(t,i)}$ will correspond to more than one mask in many other frames. 

% See the pseudo code for details.


% \begin{algorithmic}
% \State List L \Comment{stores undersegment masks}
% \For {$t=1,2,\ldots,T$}
%     \For {$i=1,2,\ldots,n_t$}
%         \State $F \gets $ frames where $M[I_{(t,i)}, :]$ is not all zero
%         \State $cnt \gets 0$, List $VF_{(t,i)}$, List $VM_{(t,i)}$
%         \For{$t' \in F$}
%             \State A $\gets$ count($M[I_{(t,i)}, t']$) \Comment{vector of how many points each mask in frame $t'$ contains}
%             \If{$A[0] < 0.7 \sum_{k} A[k]$ }
%                \State continue \Comment{most $P_{(t,i)}$ are invisible}
%             \EndIf
%             \State j = $\argmax$ A \Comment{mask id that contains most $P_{(t,i)}$}
%             \If{$A[j] > 0.9 \sum_{k} A[k] $}
%                \State $VF_{(t,i)}$.append(t')
%                \State $VM_{(t,i)}$.append((t',j))
%             \Else
%                 \State cnt += 1 \Comment{$P_{(t,i)}$ is divided into two patrs}
%             \EndIf
%         \EndFor
%         \If{$cnt > 0.1 F $}
%            \State L.append((t,i))
%         \EndIf
%     \EndFor
%  \EndFor

% \end{algorithmic}

% Now, for two candidate masks $C_{(t_1,i_1)}$ and $C_{(t_2,i_2)}$, we know that they both appear in frames $VF_{(t_1,i_1)} \cap VF_{(t_2,i_2)}$ and their third view consensus ratio is defined as, 
% \begin{equation}
%     \label{con_ratio}
%     R(C_{(t_1,i_1)}, C_{(t_2,i_2)}) = \frac{|VM_{(t_1,i_1)} \cap VM_{(t_2,i_2)}|}{|VF_{(t_1,i_1)} \cap VF_{(t_2,i_2)}|}
% \end{equation} By first converting the geometry $P_{(t,i)}$ into two simple lists, 
% $VF_{(t,i)}$ and $VM_{(t,i)}$, we avoid the heavy computation of geometry overlap between every two masks.


Though we can now merge masks with the consensus ratio, this naive method will result in severe under-segmentation, because not all edges between masks are reliable. ???

Intuitively, the more third view observers, the more reliable this consensus ratio is. Therefore, we define the confidence as the number of third view observers, i.e. $|VF_{(t_1,i_1)} \cap VF_{(t_2,i_2)}|$ and merge candidates with higher consensus ratio and higher confidence. 

In order to facilitate exposition, we define D \miyan{this word needs further consideration} as the intermediate result which contains a list of masks corresponding to the same instance. By definition, a mask can be seen as a S and our algorithm has to merge Ds into instances.

Given $D_1$ and $D_2$, we can use the same technique as \ref{con_ratio} to define the consensus ratio. Naturally, the more masks $D_i$ contains, the more complete $D_i$ is, and the more third view observers.



Then we discuss how to efficiently compute the edge weight between nodes in the new graph. Based on equation \ref{con_ratio_2}, we only need to compute $FV$ and $MC$ for each segment in this graph~\jiazhao{This should also be mentioned in the segment part. the organization of these paragraphs should be more clear.}. For each segment $S = \{m_{t_1, i_1}, m_{t_2, i_2}, \ldots, m_{t_s, i_s}\}$,~\jiazhao{$S$ is already used in L215} since its point cloud is $P'=P_{t_1,i_1}\cup P_{t_2,i_2} \ldots \cup P_{t_s, i_s}$, the frame that $S$ is visible must be the frame that at least one mask is visible and vice versa, i.e. $FV(P') = FV(P_{t_1,i_1})\cup FV(P_{t_2,i_2}) \ldots \cup FV(P_{t_s, i_s})$. As for $MC$, we use $MC(P_{t_1,i_1})\cup MC(P_{t_2,i_2}) \ldots, MC(P_{t_s, i_s})$ to approximate it because we only allow masks with high consensus ratio to be merged, which means that for frames that they both appear, they are frequently contained by a same mask at that frame, so the union of them should also be contained by this mask at that frame. \miyan{not convincing}

class-agnostic exp
\begin{table}[htbp]
\caption{\textbf{Class-agnostic mask evaluation on ScanNet200}???}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l|ccc|}
    \toprule[2pt]
    Model &    & ScanNet200&        \\ \hline
          & AP & $AP_{50}$ & $AP_{25}$ \\ \hline
          Mask3D&  39.7&        53.6&        62.5\\ \hline
          OpenMask3D &  31.3&        39.8 &        46.0\\ \hline
          OVIR-3D&    14.4&        27.5&        38.8\\ \hline
          Ours&    17.4&        33.3&        46.7\end{tabular}
}
\end{table}
